A Distinguisher-Based Attack on a Variant of McEliece's Cryptosystem Based on Reed-Solomon Codes

Baldi et \textit{al.} proposed a variant of McEliece's cryptosystem. The main idea is to replace its permutation matrix by adding to it a rank 1 matrix. The motivation for this change is twofold: it would allow the use of codes that were shown to be insecure in the original McEliece's cryptosystem, and it would reduce the key size while keeping the same security against generic decoding attacks. The authors suggest to use generalized Reed-Solomon codes instead of Goppa codes. The public code built with this method is not anymore a generalized Reed-Solomon code. On the other hand, it contains a very large secret generalized Reed-Solomon code. In this paper we present an attack that is built upon a distinguisher which is able to identify elements of this secret code. The distinguisher is constructed by considering the code generated by component-wise products of codewords of the public code (the so-called "square code"). By using square-code dimension considerations, the initial generalized Reed-Solomon code can be recovered which permits to decode any ciphertext. A similar technique has already been successful for mounting an attack against a homomorphic encryption scheme suggested by Bogdanoc et \textit{al.}. This work can be viewed as another illustration of how a distinguisher of Reed-Solomon codes can be used to devise an attack on cryptosystems based on them.

==> conclusion.tex <==
\section{Conclusion}

%The homomorphic scheme suggested in \cite{BL12} actually leads in a natural way to choose codes for which the
%square product is of  unusually small dimension, see Appendix \ref{sec:appendixB} for more details.
%This sheds some light on why considerations of this kind might lead to an attack. Replacing the Reed-Solomon codes used in the
%scheme by Reed-Muller codes does not seem to prevent this kind of attack for instance. 

%Both attacks which are presented here 
This attack may be viewed as trying to identify certain subcodes or punctured codes of the  code
used for the cryptographic scheme through square code dimension considerations
%In the Bogdanov and Lee case, this was for identifying the punctured codes with a certain number of elements of $L$ in their support. 
%In the Baldi et {\em al.} case, this was 
in order to identify codewords in a subcode of codimension $1$. Reed-Solomon codes are particularly prone to this kind of 
attack because of the very low dimension of their square code. 

The approach which is followed here seems to have other applications to cryptanalysis. For instance, it is not too difficult 
to use it for finding another way of breaking a McEliece type cryptosystem based on generalized Reed-Solomon
(the Sidelnikov-Shestakov attack \cite{SidelShesta92}) which would start by trying to identify the subcode $\GRS{k-1}{\xv}{\yv}$ of
the generalized Reed-Solomon code $\GRS{k}{\xv}{\yv}$. It might also be applied to other codes suggested in 
public key cryptosystems, such as for instance Reed-Muller codes \cite{Sid94}. The square  code of these codes have also an abnormal dimension.
The most daunting task would be to attack the McEliece cryptosystem with this kind of tools (at least in a certain range of parameters) since
the dual of Goppa codes also have in a limited way square codes with a low dimension, see  \cite{MP12a} which contains much more examples
of codes with this kind of behavior.
